Saturn: An Optimized Data System for Large Model Deep Learning Workloads

Large language models such as GPT-3 & ChatGPT have transformed deep learning (DL), powering applications that have captured the public's imagination. These models are rapidly being adopted across domains for analytics on various modalities, often by finetuning pre-trained base models. Such models need multiple GPUs due to both their size and computational load, driving the development of a bevy of "model parallelism" techniques & tools. Navigating such parallelism choices, however, is a new burden for end users of DL such as data scientists, domain scientists, etc. who may lack the necessary systems knowhow. The need for model selection, which leads to many models to train due to hyper-parameter tuning or layer-wise finetuning, compounds the situation with two more burdens: resource apportioning and scheduling. In this work, we tackle these three burdens for DL users in a unified manner by formalizing them as a joint problem that we call SPASE: Select a Parallelism, Allocate resources, and SchedulE. We propose a new information system architecture to tackle the SPASE problem holistically, representing a key step toward enabling wider adoption of large DL models. We devise an extensible template for existing parallelism schemes and combine it with an automated empirical profiler for runtime estimation. We then formulate SPASE as an MILP. We find that direct use of an MILP-solver is significantly more effective than several baseline heuristics. We optimize the system runtime further with an introspective scheduling approach. We implement all these techniques into a new data system we call Saturn. Experiments with benchmark DL workloads show that Saturn achieves 39-49% lower model selection runtimes than typical current DL practice.

==> experiments_tr.tex <==


\begin{table*}[t]
\vspace{-3mm}
\centering
\caption{Model selection configurations of workloads.}
\vspace{-3mm}
\label{table:model_selection}
%\vspace{-4mm}
\scalebox{1.0}{
\begin{tabular}{p{1.5cm} c c c c p{1.5cm} c}
\toprule
\multirow{2}{*}{Workload} & \multicolumn{5}{c}{Model Selection Configuration} & \multirow{2}{*}{\# Models}\\
\cmidrule{2-6}
 &  Model Arch. (params) & Dataset & Batch Size & Learning Rate & Epochs & \\
\midrule
TXT & {GPT-2 (1.5B), GPT-J (6B) } & WikiText-2 & \{16, 32\} & \{1e-5, 1e-4, 3e-3\} & 10 & 12\\
IMG & {ViT-G (1.8B), ResNet (200M)} & ImageNet & \{64, 128\} & \{1e-5, 1e-4, 3e-3\} & 10 & 12\\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{table*}

\section{Experimental Evaluation}\label{sec:experiments}
We now run an extensive empirical evaluation. We aim to answer two questions: (1) What performance benefits does~\system~provide compared to current practice? (2) How much do each of~\system's optimizations contribute to the overall speedups?

%\vspace{2mm}
\noindent \textbf{Workloads, Datasets, and Model Configurations:} 
We run 2 model selection workloads with benchmark DL tasks. 
Table~\ref{table:model_selection} lists the model selection configurations (neural architectures and hyper-parameters) for both workloads. 
The first (TXT) is a text workload with LLMs. It uses the popular \textit{WikiText-2}~\cite{wikitext-2} dataset. 
WikiText-2, which is drawn from Wikipedia, has previously been used as a benchmark on landmark LLMs such as GPT-2~\cite{radford2019language}.
TXT uses two GPT models: GPT-2 (1.5B parameters), introduced in 2019, and GPT-J (6B parameters), introduced in 2021. Both are still considered state-of-the-art for application-specific finetuning purposes. %\footnote{Extreme-scale LLMs such as GPT-3 or BLOOM are too large (175B+ parameters) for our current scope because they need hundreds of GPUs for reasonable runtimes, which we are unable to afford. They are likely also infeasible and/or an overkill for most end users of DL, especially in domain sciences, small companies, etc., who are our main target. We leave it to future work to extend \system~to such extreme-scale models.}
The second (IMG) is image classification comparing a large ResNet (200M parameters) and a large-scale Vision Transformer (1.8B parameters). 
It uses the computer vision benchmark dataset \textit{ImageNet}~\cite{imagenet} (14M images and 1000 classes). 
IMG's mix of model classes should help provide a more challenging workload to optimize. 

%\vspace{2mm}
\noindent \textbf{Software Setup:} 
All models are implemented and trained with PyTorch 2.0. 
We register 4 parallelisms in \system. 
\begin{enumerate}
\item PyTorch Distributed Data Parallelism~\cite{torchddp2020}.
\item PyTorch Fully-Sharded Data Parallelism~\cite{torchddp2020}.
\item GPipe, adapted from an open-source implementation~\cite{torchgpipe2020}.
\item Model spilling, provided by the FairScale library~\cite{FairScale2021}.
\end{enumerate}

We use Gurobi 10.0 for our \spase~MILP-solver; the introspection threshold and interval parameters are set to 500s and 1000s, respectively. For the underlying job orchestration, we use Ray v2.2.0. Datasets are copied across nodes upfront. 

%\vspace{2mm}
\noindent \textbf{Hardware Setup:} 
We configure 3 hardware settings: (1) 8-GPU single-node, (2) 16-GPU 2-nodes, and (3) heterogeneous 2-nodes, where one node has 8 GPUs and the other has 4 (12 GPUs in total).
All settings use machines with 1152~GB RAM, Intel Xeon 3.0~GHz 2nd Gen CPUs, a 500~GB NVMe drive, and 40~GB memory A100 GPUs connected via NVSwitch. 

%\vspace{2mm}
\noindent \textbf{Baselines:} 
No prior end-to-end system can solve the \spase~problem; prior art either does not support large models or else fails model selection constraints, as Table~\ref{tb:prior_art} showed.
So, we compare \system~with 4 baselines using the approaches in Section~\ref{sec:sched_eval}.

\begin{enumerate}
\item[(1)] \textbf{Current Practice:} A heuristic without any task parallelism within nodes. It allocates 8 GPUs per task. 
Parallelism selection is set by a human to ``optimal'' choices for an 8-GPU allocation, (typically FSDP). 
This is perhaps most representative of current practice by end users of DL. 

\item[(2)] \textbf{Random:} A randomizer tool selects parallelism and apportioning and then applies a random scheduler. This represents a system-agnostic user.

\item[(3\&4)] Two modified versions of Optimus*-Greedy (Alg. 1) combined with a randomized scheduler (see Section~\ref{sec:optimizations}). 
We name these baselines \textbf{Optimus*-Dynamic} and \textbf{Optimus*-Static}. 
These are the strongest baselines for large-model model-selection we could assemble from prior art. 
\end{enumerate}

The above approaches cover both current practices and reasonable strong heuristics for our problem setting. 
We note that the two Optimus*-based baselines use our Trial Runner as an oracle for their runtime estimates \red{and parallelism selection decisions} (the original Optimus paper only had runtime models for Parameter Server-style data parallelism~\cite{peng2018optimus}). 
This highlights the novelty of our problem setting --- the strongest baseline from prior art needs to reuse a module of our system.

%We originally planned on including Pollux~\cite{qiao2021pollux} as another baseline.
%Unfortunately, we found that adapting Pollux to support multiple techniques and large-model training would require significant implementation effort.
%Moreover, one of their key performance optimizations (DL workload knob tuning) is antithetical to the purpose of model selection.
%Pollux's aims are fundamentally different from our own; redesigning it for our setting would involve creating a new system altogether.
%Since a re-designed/engineered Pollux baseline would not be a good representation of existing practice, we exclude it.

\subsection{End-to-End Results}\label{sec:experiments_end_to_end}

\begin{figure*}[t]
\includegraphics[width=0.9\textwidth]{images/e2e_panel_revision.pdf}
\vspace{-6mm}
\caption{(A) End-to-end runtimes. Speedups versus current practice are also noted. Results are averaged over three trials, with the 90\% confidence interval displayed.
(B) Average GPU utilization over time at a 100s sampling rate on the single-node TXT job. (C) End-to-end runtimes of \system~versus compositions of tools on a reduced version of the TXT job on 2 nodes.}
\label{fig:e2e}
\vspace{-2mm}
\end{figure*}

%\vspace{1mm}
\noindent \textbf{Model Selection Runtimes:} 
We first compare the end-to-end runtimes versus the 4 baselines. 
The Trial Runner search overheads are \textit{included} in \system's runtime.
Figure~\ref{fig:e2e}(A) presents the results. 
%(C) also illustrates our system's \spase~solution for the single-node TXT workload. 
%Our tech report~\cite{techreport} provides the other solutions.

\system~achieves significant speedups versus all baselines.
Against Current Practice, we see makespan reductions of 39-40\% on a single-node, 43-48\% on 2 homogeneous nodes, and 41-45\% on 2 heterogeneous nodes.
Against the strongest baseline (Optimus*-Dynamic), we see makespan reductions of 30-34\%, 38-40\%, and 32-39\% on the three hardware configurations respectively.
Since the same UPP implementations are used \textit{in all cases}, the speedups are achieved purely via the better parallelism selections, resource allocations, and schedule constructions. 
All compared approaches (including \system) use logically equivalent SGD and offer the same accuracy. 

Figure~\ref{fig:e2e}(B) plots GPU utilization.
%All baselines use the same underlying parallelism implementations, so this metric is fairly consistent across approaches.
\system~achieves good utilization throughout, except an initial low-utilization period for the Trial Runner's search and MILP solving period. 
%We attribute this to \system's well-selected \spase~solution, which reduces idle times with effective resource apportioning and parallelism selection.
GPU utilization alone can be misleading; tools such as nvidia-smi can artificially inflate utilization~\cite{nvidiasmi}. So, these results should not be taken as a measure of training performance in isolation.

Overall,~\system~reduces model selection runtimes substantially for all workloads in all evaluated settings. 
It also offers more qualitative benefits to end users of DL because they are freed from manually selecting parallelisms, deciding on resource allocations, or tuning system parameters.

%\vspace{1mm}
\noindent \textbf{Intuition on Efficiency Gains.} 
\system's performance improvements arise due to its \textit{holistic} optimization approach. 
To the best of our knowledge, this is the first work that characterizes the parallelism performance crossovers and incorporates them into a joint optimizer.
Our empirical profiler and unified \spase~formulation enable us to optimize in a parallelism-agnostic fashion. 
The heuristic and algorithmic baselines make assumptions about scaling behaviors (e.g., consistency, linear scaling, etc.) that do not always hold up in large-model DL practice. 
To prove our point further, Table~\ref{table:selected_outputs} lists the parallelisms+allocations selected by \system~for a few models from the single-node workloads. We see a non-trivial mixture of decisions across the models trained.

\begin{table}[h]
\vspace{-1mm}
\centering
\caption{Parallelisms and apportionments chosen by \system~for a few evaluated models.}
\label{table:selected_outputs}
\vspace{-4mm}
\begin{tabular}{clclc}
\toprule
Model Config & Parallelism & Apportionment\\
\midrule
GPT-2 (Batch 16, 1e-5 LR) & Pipelining & 5 GPUs \\
GPT-2 (Batch 32, 1e-4 LR) & FSDP & 4 GPUs\\
GPT-J (Batch 16, 1e-5 LR) & FSDP & 8 GPUs\\
GPT-J (Batch 32, 1e-4 LR) & Pipelining & 3 GPUs \\
ResNet (Batch 64, 1e-4 LR) & DDP & 2 GPUs \\
ResNet (Batch 32, 1e-4 LR) & Spilling & 1 GPU\\
ViT-G (Batch 32, 1e-4 LR) & FSDP & 4 GPUs\\
ViT-G (Batch 16, 1e-4 LR) & FSDP & 6 GPUs\\
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

\system's MILP-chosen \spase~solutions may seem unintuitive individually, but they combine into a multi-model \spase~solution to minimize end-to-end runtimes.
It is unreasonable to expect practitioners to have the systems knowhow to manually design such a complex mix. 
Our unified data systems-style approach frees DL users to focus on their goals instead of tedious low-level decisions. 

{\color{red}
\subsection{Joint Optimization Evaluation}
To better understand the value of joint optimization for \spase, we evaluate \system~against different compositions of tools --- Alpa~\cite{alpa2022} + ASHA~\cite{asha2018};  Alpa + Optimus*~\cite{peng2018optimus}; Alpa + SHA~\cite{hyperband} --- each used together but unaware of each other. We note that it is non-trivial for regular DL users to implement such compositions, but these baselines can help elucidate the value of joint optimization. A/SHA \& Optimus are designed for multi-model training and GPU allocation; Alpa tackles parallelism selection. In combination, they can be used to solve the dimensions of the \spase~problem, but in a separated fashion. We elaborate on these tools in Section \ref{sec:related_work}.

To mimic A/SHA's early-stopping behaviors, we run \system~and Optimus* one epoch at a time. We take the early stops produced by A/SHA and apply them to \system~and Optimus*'s workloads on epoch boundaries.
A/SHA is configured to use 3 rungs, with allocations of 1, 3, and 6 epochs respectively, so completed jobs will have run for 10 epochs.
The decay factor is set to 2, so half of the jobs survive each rung. 
Since A/SHA was built for settings with substantially more accelerators than models, we use a smaller version of the TXT workload with 8 jobs (eliminating the 3e-3 learning rate option) on 2 nodes.
This lets us present the A/SHA baseline in the most favorable light feasible.

We report the results in Figure~\ref{fig:e2e}(C). We find that \system~outperforms Alpa + ASHA by nearly 3X. Even if we remove Alpa's search times (e.g., if the searches were run once up-front) and directly compare \spase~solution quality, \system~still outperforms the composite baseline by 1.67X. Against Alpa + Optimus*, the speedups are 6.25X (resp. 1.54X) when including (resp. excluding) Alpa's compilation times. The Optimus* runtime that includes the compilation times is so high because it needs to construct its throughput oracle~\cite{qiao2021pollux} up front by running the compiler for every possible allocation for every model. \system's significant speedups against all 3 baselines support our view that the \spase~problem is a novel space where joint optimization has a significant role to play, rather than a simple composition of existing problem spaces.
}

\subsection{Drilldown Analyses}\label{sec:ablation}

%\vspace{1mm}
\subsubsection{\textbf{Ablation Study}}  We separate our optimizations into 4 layers: scheduling, resource allocation, parallelism selection, and introspection. 
We apply these one-by-one as follows. 
First, a version without any of our optimizations. FSDP is used with checkpointing and offloading (i.e., a non-expert config), resource allocations are set manually to 4 GPUs per task, and a random scheduler is used.
Second, we use our makespan-optimized scheduler. %This illustrates performance against against makespan-optimized schedulers that lack parallelism selection + resource allocation capabilities (e.g. Gavel~\cite{gavel2020}).
Third, we reintroduce resource apportioning to the MILP.
Fourth, we allow for automatic parallelism selection and knob tuning.
Finally, we overlay introspection. This completes~\system.
We use the single-node TXT workload in our study.
%The use of a makespan-optimized MILP offers a ~1.1X speedup; it degenerates into an instance of the Longest-Job-First approximation for multiset partitioning jobs.
%Resource scheduling provides a ~1.2X marginal speedup. With this, the system can now choose how to balance between task parallelism (fewer resources per job) and local techniques.
%Automatic technique selection/tuning provides a substantial marginal speedup of ~1.5X. As shown in prior art and in our crossover diagrams, choosing the right technique and tuning it correctly can improve performance significantly~\cite{terapipe2021}.
%Introspection provides a ~1.15X marginal speedup. 
Table~\ref{tb:ablation} notes the marginal speedups.

\begin{table}[h]
\centering
\vspace{-3mm}
\caption{Ablation study.}
\label{tb:ablation}
\vspace{-4mm}
\begin{tabular}{clclc}
\toprule
Optimizations & Abs. Speedup & Extra Speedup\\
\midrule
Unoptimized & 1.0X & 1.0X\\
+ MILP Scheduler & 1.1X & 1.1X\\
+ Resource Allocation in MILP & 1.33X & 1.2X\\
+ Auto. Parallelism Selection & 1.95X & 1.47X \\
+ Introspection & 2.27X & 1.16X \\
\bottomrule
\end{tabular}
\vspace{-1mm}
\end{table}

The scheduler-only MILP provides better packing for some initial makespan improvements. 
Adding in resource apportioning lets the solver reshape task runtimes and demands to produce more speedups. 
Automatic parallelism selection creates even more flexibility and adds in knob-tuning to improve parallelism performance. Introspection enables the solver to reassess its solution and adapt to shifts in the workload to cap off \system's speedups.

\begin{figure}
\includegraphics[width=\columnwidth]{images/opt_panel_small.pdf}
\vspace{-6mm}
\caption{\system~sensitivity plots on the TXT workload versus (A) workload size, (B) model size, and (C) node size. Charts are in log-log scales, normalized to the initial setting. (C) labels each point with the marginal speedup.}
\label{fig:opt}
\vspace{-5mm}
\end{figure}

\subsubsection{\textbf{Sensitivity Analyses}} We test \system's sensitivity to the size of: (1) workloads, (2) models, and (3) clusters. 

For workload size scaling, we run TXT on a single 8-GPU node with the GPT-2 model, set batch size to 16, and vary the number of learning rates explored. Figure~\ref{fig:opt}(A) presents the results.
\system~scales slightly superlinearly as larger workloads enable broader scope for optimization.
This suggests strong performance on large-scale model selection workloads.

Next, we vary model size. We run TXT on a single 8-GPU node with batch size set to 16 and learning rate set to 1e-5.
All models are versions of GPT-2. We vary model size by stacking encoder blocks, akin to what GPT-3 does~\cite{gpt2020}. Figure~\ref{fig:opt}(B) presents the results.
\system~achieves mostly linear scaling, but with slight slowdowns on the largest model sizes. 
This is because the largest models force the \spase~solution to use the only viable configuration (8-GPU FSDP with checkpointing and offloading) for every model. 
%This study shows how our \system's performance can be limited by the underlying UPP implementations; while it can solve \spase~effectively, it still needs performant UPP options.

Finally, we vary the number of GPUs visible to~\system. We switch to 2 nodes for the 16-GPU case.
We use TXT for this experiment. Figure~\ref{fig:opt}(C) presents the results.
\system~achieves superlinear speedups. We suggest 2 causes. 
First, the single-GPU case necessitates DRAM spilling, while larger GPU counts reduce the degree of spilling required and open a larger space of parallelisms. 
Second, higher GPU counts broaden the solution space for the MILP, enabling higher flexibility,
%Note that this particular analysis is more reflective of how our UPP implementations perform rather than the actual system.

